Globally Optimal Multi-Scale Monocular Hand-Eye Calibration Using Dual Quaternions

In this work, we present an approach for monocular hand-eye calibration from per-sensor ego-motion based on dual quaternions. Due to non-metrically scaled translations of monocular odometry, a scaling factor has to be estimated in addition to the rotation and translation calibration. For this, we derive a quadratically constrained quadratic program that allows a combined estimation of all extrinsic calibration parameters. Using dual quaternions leads to low run-times due to their compact representation. Our problem formulation further allows to estimate multiple scalings simultaneously for different sequences of the same sensor setup. Based on our problem formulation, we derive both, a fast local and a globally optimal solving approach. Finally, our algorithms are evaluated and compared to state-of-the-art approaches on simulated and real-world data, e.g., the EuRoC MAV dataset.

==> tables/substitution.tex <==
\newcommand{\nn}[0]{$\pm$}
\newcommand{\zero}[1]{$s_{#1} = 0$}
\newcommand{\fraction}[2]{$\dfrac{s_{#1}}{r_{#1}} = \dfrac{s_{#2}}{r_{#2}}$}

\renewcommand{\arraystretch}{2}
\begin{tabular}{cccc|cccccc}
    \toprule
    
    \multicolumn{4}{c}{\textbf{Rotation}} & \multicolumn{6}{c}{\textbf{Constraint}} \\
    
    $r_1$ & $r_2$ & $r_3$ & $r_4$ &
    $r_1 s_2 = r_2 s_1$ & $r_1 s_3 = r_3 s_1$ & $r_1 s_4 = r_4 s_1$ &
    $r_2 s_3 = r_3 s_2$ & $r_2 s_4 = r_4 s_2$ & $r_3 s_4 = r_4 s_3$ \\
    
    \midrule
    
    0 & 0 & 0 & 0 &
    -- & -- & -- &
    -- & -- & -- \\
    
    0 & 0 & 0 & \nn &
    -- & -- & \zero{1} &
    -- & \zero{2} & \zero{3} \\
    
    0 & 0 & \nn & 0 &
    -- & \zero{1} & -- &
    \zero{2} & -- & \zero{4} \\
    
    0 & 0 & \nn & \nn &
    -- & \zero{1} & \zero{1} &
    \zero{2} & \zero{2} & \fraction{3}{4} \\
    
    0 & \nn & 0 & 0 &
    \zero{1} & -- & -- &
    \zero{3} & \zero{4} & -- \\
    
    0 & \nn & 0 & \nn &
    \zero{1} & -- & \zero{1} &
    \zero{3} & \fraction{2}{4} & \zero{3} \\
    
    0 & \nn & \nn & 0 &
    \zero{1} & \zero{1} & -- &
    \fraction{2}{3} & \zero{4} & \zero{4} \\
    
    0 & \nn & \nn & \nn &
    \zero{1} & \zero{1} & \zero{1} &
    \fraction{2}{3} & \fraction{2}{4} & \fraction{3}{4} \\
    
    \nn & 0 & 0 & 0 &
    \zero{2} & \zero{3} & \zero{4} &
    -- & -- & -- \\
    
    \nn & 0 & 0 & \nn &
    \zero{2} & \zero{3} & \fraction{1}{4} &
    -- & \zero{2} & \zero{3} \\
    
    \nn & 0 & \nn & 0 &
    \zero{2} & \fraction{1}{3} & \zero{4} &
    \zero{2} & -- & \zero{4} \\
    
    \nn & 0 & \nn & \nn &
    \zero{2} & \fraction{1}{3} & \fraction{1}{4} &
    \zero{2} & \zero{2} & \fraction{3}{4} \\
    
    \nn & \nn & 0 & 0 &
    \fraction{1}{2} & \zero{3} & \zero{4} &
    \zero{3} & \zero{4} & -- \\
    
    \nn & \nn & 0 & \nn &
    \fraction{1}{2} & \zero{3} & \fraction{1}{4} &
    \zero{3} & \fraction{2}{4} & \zero{3} \\
    
    \nn & \nn & \nn & 0 &
    \fraction{1}{2} & \fraction{1}{3} & \zero{4} &
    \fraction{2}{3} & \zero{4} & \zero{4} \\
    
    \nn & \nn & \nn & \nn &
    \fraction{1}{2} & \fraction{1}{3} & \fraction{1}{4} &
    \fraction{2}{3} & \fraction{2}{4} & \fraction{3}{4} \\
    
    \bottomrule    
\end{tabular}
